Compressing 3D Gaussian Splatting by Noise-Substituted Vector Quantization

3D Gaussian Splatting (3DGS) has demonstrated remarkable effectiveness in 3D reconstruction, achieving high-quality results with real-time radiance field rendering. However, a key challenge is the substantial storage cost: reconstructing a single scene typically requires millions of Gaussian splats, each represented by 59 floating-point parameters, resulting in approximately 1 GB of memory. To address this challenge, we propose a compression method by building separate attribute codebooks and storing only discrete code indices. Specifically, we employ noise-substituted vector quantization technique to jointly train the codebooks and model features, ensuring consistency between gradient descent optimization and parameter discretization. Our method reduces the memory consumption efficiently (around $45\times$) while maintaining competitive reconstruction quality on standard 3D benchmark scenes. Experiments on different codebook sizes show the trade-off between compression ratio and image quality. Furthermore, the trained compressed model remains fully compatible with popular 3DGS viewers and enables faster rendering speed, making it well-suited for practical applications.

==> fig/fig_tex/qualitative_all_scenes.tex <==
%% Qualitive comparison 
\begin{figure*}[!t]
  \centering
  % Column titles
  \hspace*{0.03\textwidth}
  \foreach \method [count=\i] in {{Ground truth},{3DGS},{CompGS (16k)},{\modelname\ (16k)}}{
    \begin{subfigure}[c]{0.22\textwidth}
      \centering\strut\method
    \end{subfigure}
  }
  % Removed to save space: counter, drjohnson, bicycle, bonsai, garden,
  \foreach \scene [count=\j] in {flowers, treehill, drjohnson, kitchen, bonsai, train, truck} {
  \begin{tabular}{c}
    \begin{subfigure}[c]{0.03\textwidth}
      \tikz\node[rotate=90,font=\sc\strut]{\scene};
    \end{subfigure}
    \foreach \method [count=\i] in {gt,3dgs,compgs16k,newvq16k}{
      \begin{subfigure}[c]{0.22\textwidth} % Each figure takes 1/4th of text width
        \centering
        \includegraphics[width=\textwidth]{fig/qualitative_all_scenes/\scene_\method}
      \end{subfigure}
      \vspace*{-1pt}
    }
  \end{tabular}\\[.5em]
  }
  \vspace*{-.1in}
  \caption{Qualitative comparison between ground truth, 3DGS, CompGS (16k), and \modelname\ (16k) (ours).}
\label{fig:qualitative_allscenes}
  \vspace*{-.1in}
\end{figure*}

==> fig/fig_tex/qualitative_half_thousand.tex <==
%% Qualitive comparison 
\begin{figure*}[t]
  \raggedleft
  \setlength{\figurewidth}{0.23\textwidth}
  \setlength{\figureheight}{\figurewidth}
  \foreach \method/\methodname [count=\j] in {gt/{\strut Ground truth},compgs0.5k/{\strut ~CompGS\ (0.5k)~}, newvq0.5k/{\strut \modelname\ (0.5k)}} {
  \begin{tikzpicture}[
      image/.style = {inner sep=0pt, outer sep=0pt, 
        minimum width=.95\figurewidth, anchor=north west, text width=.95\figurewidth}, 
      node distance = 1pt and 1pt, every node/.style={font= {\tiny}}, 
      label/.style = {font={\strut\footnotesize\bf},anchor=south,inner sep=0pt}, 
      spy using outlines={rectangle, magnification=1, size=0.475\figurewidth}
    ] 

    % \foreach \method [count=\j] in {newvq0.5k,gt} {
    % Loop over scenes
    \foreach \scene [count=\i] in {bicycle,bonsai,counter,garden} {
      % The actual image
      \node[image] (img-\i) at (\i*\figurewidth,0) 
        {\includegraphics[width=.95\figurewidth]{fig/qualitative_half_thousand/\scene_\method}};
        
      % Label top
      \ifnum\j=1
        \node[anchor=south,font=\strut\sc] at (img-\i.north) {\scene};
      \fi
      
      % Label left
      \ifnum\i=1
        \node[anchor=south,font=\strut,rotate=90,anchor=south] at (img-\i.west) {\methodname};
      \fi
      
        
      % Set coordinates
      \coordinate (spypoint-\i-a) at ($(img-\i.south west)$);
      \coordinate (spypoint-\i-b) at ($(img-\i.south east)$);      
      
    }
    
    % Set spy coordinates (1a)
    \coordinate (spot-1-a) 
      at ($(img-1.south west) + (0.3\figurewidth,.4\figurewidth)$); % <- EDIT
    \spy[white,magnification=2] on 
      (spot-1-a) in node[anchor=north west] at (spypoint-1-a);
    % Set spy coordinates (1b) 
    \coordinate (spot-1-b) 
      at ($(img-1.south west) + (0.6\figurewidth,.3\figurewidth)$); % <- EDIT
    \spy[white,magnification=4] on 
      (spot-1-b) in node[anchor=north east] at (spypoint-1-b);
    
    % Set spy coordinates (2a)
    \coordinate (spot-2-a) 
      at ($(img-2.south west) + (0.08\figurewidth,.55\figurewidth)$); % <- EDIT
    \spy[white,magnification=4] on 
      (spot-2-a) in node[anchor=north west] at (spypoint-2-a);
    % Set spy coordinates (2b) 
    \coordinate (spot-2-b) 
      at ($(img-2.south west) + (0.55\figurewidth,.4\figurewidth)$); % <- EDIT
    \spy[white,magnification=1.5] on 
      (spot-2-b) in node[anchor=north east] at (spypoint-2-b);  
      
    % Set spy coordinates (3a)
    \coordinate (spot-3-a) 
      at ($(img-3.south west) + (0.08\figurewidth,.55\figurewidth)$); % <- EDIT
    \spy[white,magnification=4] on 
      (spot-3-a) in node[anchor=north west] at (spypoint-3-a);
    % Set spy coordinates (3b) 
    \coordinate (spot-3-b) 
      at ($(img-3.south west) + (0.6\figurewidth,.3\figurewidth)$); % <- EDIT
    \spy[white,magnification=1.5] on 
      (spot-3-b) in node[anchor=north east] at (spypoint-3-b);   
      
    % Set spy coordinates (4a)
    \coordinate (spot-4-a) 
      at ($(img-4.south west) + (0.1\figurewidth,.5\figurewidth)$); % <- EDIT
    \spy[white,magnification=4] on 
      (spot-4-a) in node[anchor=north west] at (spypoint-4-a);
    % Set spy coordinates (4b) 
    \coordinate (spot-4-b) 
      at ($(img-4.south west) + (0.5\figurewidth,.4\figurewidth)$); % <- EDIT
    \spy[white,magnification=2] on 
      (spot-4-b) in node[anchor=north east] at (spypoint-4-b);
      
  \end{tikzpicture}~~~\\[-8pt]
  %\vspace*{-8pt}
  }    
  \vspace*{.05in}
  \caption{
    Qualitative comparison between ground truth, CompGS (0.5k), and \modelname\ (0.5k) (ours). Our \modelname\ captures difficult sharp boundaries and straight lines better compared to CompGS (see, \eg, {\sc bicycle}). This becomes clearer at stronger compression constraints (low codebook bitrates).}
  \label{fig:qualitative_0.5k}
  \vspace*{-.1in}
\end{figure*}

==> fig/fig_tex/scatter-size_metrics.tex <==
\begin{figure}[t!]
  \centering\small
  \setlength{\figurewidth}{.6\textwidth}
  \setlength{\figureheight}{.6\textwidth}
  \pgfplotsset{
    y tick label style={rotate=90},
    semithick/.append style={line width=3pt,opacity=.8},
    legend style={font=\footnotesize},
    ylabel style={font=\large},
    xlabel style={font=\large},
    grid style={dashed,lightgray},
    legend style={draw=none,inner xsep=2pt, inner ysep=0.5pt, nodes={inner sep=1.5pt, text depth=0.1em},fill=white,fill opacity=0.8}
    %every axis plot/.append style={forget plot}
    }
  \foreach \dataset/\nicename [count=\j] in {MipNeRF360/{Mip-NeRF 360}, TanksAndTemples/{Tanks and Temples}, DeepBlending/{Deep Blending}} {
    % Title
    \begin{subfigure}[b]{0.02\textwidth}
      \centering 
      \tikz\node[rotate=90,text width=.62\figureheight,align=center,font=\bf\strut,scale=.8]{\nicename};
    \end{subfigure}%
    %
    \foreach \metric [count=\i] in {PSNR, SSIM, LPIPS} {
      \begin{subfigure}[b]{0.31\textwidth}
        \raggedleft 
        \scalebox{.5}{\input{fig/scatter-size_metrics/\dataset_\metric.tex}}
      \end{subfigure}
  }}
  \vspace*{-1.5em}
  \definecolor{steelblue31119180}{RGB}{31,119,180}
  \definecolor{lightgrey}{RGB}{211,211,211}
  \caption{The comparison of reconstruction quality across baselines. In each sub-figure, the $x$-axis denotes the model size in Megabytes, $y$-axis denotes the metrics on the reconstruction result. Each method comprising different sub-methods is plotted as multiple connected points. Our \textcolor{steelblue31119180}{\textbf{\modelname}}\ performs best within the category of SP-based methods, whereas ML-based methods (in \textcolor{lightgrey}{\bf gray}) can boost performance further while losing some of the appealing 3DGS propeties.   \looseness-1
  %The three columns refers to datasets Mip-NeRF360, Deep Blending and Tanks \& Temples from left to right respectively, the three rows refers to the PSNR, SSIM, LPIPS from top to bottom respectively 
  }
  \label{fig:quantitative_scatter}
\end{figure}

==> table/reconstruction_benchmark.tex <==
\begin{tabular}{ll|cccc|cccc|cccc}
\toprule
 && \multicolumn{4}{c}{Mip-NeRF 360} & \multicolumn{4}{c}{Tanks and Temples} & \multicolumn{4}{c}{Deep Blending}
\\ 
   &Methods & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & Size$\downarrow$ &PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & Size$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & Size$\downarrow$
\\\midrule
\rowcolor{blue!10} &\modelname\ (16k) (ours) & \boldvalue{27.28} & 0.807 & 0.239 & \boldvalue{16.38} & \boldvalue{23.62} & \boldvalue{0.842} & 0.190 & \boldvalue{11.02} & \boldvalue{29.90} & \boldvalue{0.906} & \boldvalue{0.249} & \boldvalue{11.49} \\
&CompGS (16k) & 27.03 & 0.804 & 0.243 & 18 & 23.39 & 0.836 & 0.200 & 12 & \boldvalue{29.90} & \boldvalue{0.906} & 0.252 & 12 \\
&Reduced3DGS & 27.10 & \boldvalue{0.809} & \boldvalue{0.226} & 29 & 23.57 & 0.840 & \boldvalue{0.188} & 14 & 29.63 & 0.902 & \boldvalue{0.249} & 18 \\
&Compact3DGS & 27.08 & 0.798 & 0.247 & 48.8 & 23.32 & 0.831 & 0.201 & 39.4 & 29.79 & 0.901 & 0.258 & 43.2 \\
&LightGaussians & \boldvalue{27.28} & 0.805 & 0.243 & 42 & 23.11 & 0.817 & 0.231 & 22 & \nan & \nan & \nan & \nan \\
\rotate{-6}{SP-based}\cellcolor{white}&Compressed3D & 26.98 & 0.801 & 0.238 & 28.8 & 23.32 & 0.832 & 0.194 & 17.28 & 29.38 & 0.898 & 0.253 & 25.3 \\
\midrule
\rotate{3}{ML-based} &HAC (lowrate) & 27.53 & 0.807 & 0.238 & 15.26 & 24.04 & 0.846 & 0.187 & 8.1 & 29.98 & 0.902 & 0.269 & 4.35 \\
&SOG & 27.08 & 0.799 & 0.230 & 38.42 & 23.56 & 0.837 & 0.186 & 21.72 & 29.26 & 0.894 & 0.268 & 16.92 \\
&ContextGS (lowrate) & 27.62 & 0.808 & 0.237 & 12.68 & 24.12 & 0.849 & 0.186 & 9.443 & 30.09 & 0.907 & 0.265 & 3.485 \\
\midrule
 &3DGS & 27.21 & 0.815 & 0.214 & 734 & 23.14 & 0.841 & 0.183 & 411 & 29.41 & 0.903 & 0.243 & 676 \\
\bottomrule
\end{tabular}
